Path instability of deformable bubbles rising in Newtonian liquids: A linear study

The first stages of the path instability phenomenon known to affect the buoyancy-driven motion of gas bubbles rising in weakly or moderately viscous liquids are examined thanks to a recently developed numerical tool designed to assess the global linear stability of incompressible flows involving freely-evolving interfaces. Predictions for the critical bubble size and frequency of the most unstable mode are found to agree well with reference data obtained in ultrapure water and in several silicone oils. By varying the bubble size, stability diagrams are built for several specific fluids, revealing three distinct regimes characterized by different bifurcation sequences. The spatial structure of the corresponding unstable modes is analysed, together with the variations of the bubble shape, position and orientation. For this purpose, displacements of the bubble surface are split into rigid-body components and volume-preserving deformations, allowing us to determine how the relative magnitude of the latter varies with the fluid properties and bubble size. Predictions obtained with freely-deformable bubbles are compared with those found when the bubble shape determined in the base state is constrained to remain frozen during the stability analysis. This comparison reveals that deformations leave the phenomenology of the first bifurcations unchanged in low-viscosity fluids, especially water, only lowering the critical bubble size and increasing the frequency of path oscillations. In contrast, they introduce a dramatic change in the nature of the primary bifurcation in oils slightly more viscous than water, whereas, somewhat surprisingly, they leave the near-threshold phenomenology unchanged in more viscous oils.

==> custom.tex <==

\usepackage{hyperref}
%\usepackage[dvipsnames]{xcolor}
\usepackage[x11names]{xcolor}


\usepackage{graphicx}
\usepackage{tikz}
\usepackage{epstopdf, epsfig}

\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}


%%% FROM PAUL

\usepackage{subfig}
\usepackage{wrapfig}
\usepackage{multirow}


%\hypersetup{
%    colorlinks,
 %   citecolor=black,
 %   filecolor=black,
  %  linkcolor=black,
   % urlcolor=black
%}

%\PassOptionsToPackage{francais}{babel} % change this to your language(s), main language last
% Spanish languages need extra options in order to work with this template
%\PassOptionsToPackage{spanish,es-lcroman}{babel}
 %   \usepackage{babel}


%%%%%%% MACROS FROM PAUL

\newcommand{\vect}[1]{\overrightarrow{#1}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\vsigb}{\boldsymbol{\varsigma}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\sigmab}{\boldsymbol{\sigma}}
\newcommand{\psib}{\boldsymbol{\psi}}
\newcommand{\phib}{\boldsymbol{\varphi}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\sg}{\boldsymbol{\sigma}}
\newcommand{\gd}[1]{\mathlarger{\mathlarger{\mathlarger{#1}}} }
\newcommand{\ptit}[1]{\mathsmaller{\mathsmaller{\mathsmaller{{#1}}}}}
\newcommand{\gdpt}[2]{\mathlarger{\mathlarger{\mathlarger{#1}}}
_{{#2}} }
\newcommand{\Gdpt}[2]{\larger{\larger{\larger{\larger{#1}}}}
_{\smaller{\smaller{\smaller{{{#2}}}}}}}

\newcommand{\tens}[1]{\boldsymbol{\bar{\bar{#1}}}}
\newcommand{\hatf}[1]{\widehat{\boldsymbol{#1}}}
\newcommand{\hatfp}[1]{\widehat{\boldsymbol{#1}'}}

\newcommand{\R}{\mathbf{x}_0+\epsilon\xib}
\newcommand{\RR}{\mathbf{x}_0}
\newcommand{\devU}{\mathbf{u}(\RR)+\epsilon\boldsymbol{\eta}.\nabla_{\Omega_0}\mathbf{u}(\RR)}
\newcommand{\Ulin}{\mathbf{u}_0(\RR)+\epsilon\mathbf{u}_1(\RR,t)}
\newcommand{\Plin}{p_0(\RR)+\epsilon p_1(\RR,t)}
\newcommand{\ulin}{\mathbf{u}_0+\epsilon\mathbf{u}_1}
\newcommand{\plin}{p_0+\epsilon p_1}

\newcommand{\tr}{\mathrm{Tr}}

\newcommand{\pe}{\hat{p}_1}
\newcommand{\Sigmae}{\hat{\Sigma}_1}
\newcommand{\etae}{\hat{\eta}}
\newcommand{\ue}{\hat{\textbf{u}}_1}
\newcommand{\qe}{\hat{\textbf{q}}_1}
\newcommand{\Ne}{\hat{\textbf{n}}_1}
\newcommand{\ke}{\hat{\kappa}_1}
\newcommand{\pbe}{\hat{p}_{b_1}}
\newcommand{\xibe}{\hat{\xib}}
\newcommand{\xibbe}{\hat{\xib}_b}

\newcommand{\expi}{e^{\lambda + im\varphi_0}}
\newcommand{\Omegate}{{\Omega_{t^*}}}
\newcommand{\Omegat}{{\Omega_{t}}}
\newcommand{\Omegaz}{{\Omega_0}}
%\newcommand{\nablat}{\nabla_{\Omega_t}}
%\newcommand{\nablaz}{\nabla_{\Omega_0}}
\newcommand{\nablat}{\nabla}
\newcommand{\nablaz}{\nabla_0}
\newcommand{\Gammabz}{{\Gamma_{b_0}}}
\newcommand{\Omegabz}{{\Omega_{b_0}}}
\newcommand{\Gammab}{{\Gamma_b}}

\newcommand{\deriv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\ddt}[1]{\frac{\partial #1}{\partial t}}

\newcommand{\be}[1]{\begin{equation} \label{#1}}
\newcommand{\ee}{\end{equation}}

\newcommand{\GdOepsi}{{\cal O}(\epsilon^2)}  
\newcommand{\eqref}[1]{\ref{#1}}


%\usepackage{color}

%%%%%%%% MACROS FROM DAVID WITH COLORS

\newcommand{\qf}{{\color{blue} {\bf q}_f}}
\newcommand{\qzero}{{\color{blue} {\mathbf q}_{f,0}}}
\newcommand{\uzero}{{\color{blue} {\mathbf u}_0}}
\newcommand{\pzero}{{\color{blue} p_0}}
\newcommand{\nzero}{{\color{blue} {\mathbf n}_0}}
\newcommand{\tzero}{{\color{blue} {\mathbf t}_0}}
\newcommand{\kappazero}{{\color{blue} \kappa_0}}
\newcommand{\Omegazero}{{\color{blue} \Omega_0}}
\newcommand{\Gammabzero}{{\color{blue} \Gamma_{b0}}}
\newcommand{\xzero}{{\color{blue} \mathbf{x}_0}}
\newcommand{\xz}{{\color{blue} \mathbf{x}_0}}
\newcommand{\x}{\mathbf{x}}

\newcommand{\qone}{{\color{green} {\mathbf q}_{f,1}}}
\newcommand{\uone}{{\color{green} {\mathbf u}_1}}
\newcommand{\pone}{{\color{green} p_1}}

\newcommand{\xione}{{\color{magenta} \xib}}

\newcommand{\etaone}{{\color{red} \eta}}
\newcommand{\none}{{\color{red} {\mathbf n}_1}}
\newcommand{\tone}{{\color{red} {\mathbf t}_1}}
\newcommand{\kappaone}{{\color{red} \kappa_1}}

\newcommand{\ubone}{{\color{orange} u_{b1}}}
\newcommand{\pgone}{{\color{orange} p_{g1}}}


\newcommand{\qmode}{{\color{green} \hat{\mathbf q}_1}}
\newcommand{\umode}{{\color{green} \hat{\mathbf u}_1}}
\newcommand{\pmode}{{\color{green} \hat{p_1}}}

\newcommand{\ximode}{{\color{magenta} \hat{\xib}}}

\newcommand{\etamode}{{\color{red} \hat{\eta}}}
\newcommand{\nmode}{{\color{red} \hat{\mathbf n}_1}}
\newcommand{\tmode}{{\color{red} \hat{\mathbf t}_1}}
\newcommand{\kappamode}{{\color{red} \hat{\kappa_1}}}

%%%%%% MACROS INTRODUCED BY DAVID : TEST FUNCTIONS
\newcommand{\qftest}{\tilde{\mathbf{q}_f}}
\newcommand{\utest}{\tilde{\mathbf{u}}}
\newcommand{\ptest}{\tilde{p}}
\newcommand{\xitest}{\tilde{\mathbf{\xib}}}
\newcommand{\etatest}{\tilde{\eta}}
\newcommand{\ktest}{\tilde{\kappa}}
\newcommand{\pbtest}{\tilde{p_b}}

%\newcommand{\cadrebleu}[1]{
%\begin{mdframed}[style=mdstyle1]
%{#1}
%\end{mdframed}}

%\newcommand{\cadre}[3]{
%\begin{mdframed}[backgroundcolor={#1}!{#2}]
%{#3}
%\end{mdframed}}

\newcommand{\cadrebleu}[1]{#1}

\newcommand{\cadre}[3]{#3}

\newcommand{\citer}[1]{\cite{ #1}}
\newcommand{\text}[1]{\mbox{ #1}}

\usepackage{tikz,tikz-3dplot,pgfplots}
\usetikzlibrary{shapes,arrows}
\usepackage{lscape}
\usepackage[framemethod=TikZ]{mdframed}
\usepackage{wrapfig}

